Soil Sample Search in Partially Observable Environments

To work in unknown outdoor environments, autonomous sampling machines need the ability to target samples despite limited visibility and robotic arm reach distance. We design a heuristic guided search method to speed up the search process and more efficiently localize the approximate center of soil regions. Through simulation experiments, we assess the effectiveness of the proposed algorithm and discover superior performance in terms of speed, distance traveled, and success rate compared to naive baselines.

==> Soil_Sample_Search_in_a_Partially_Observable_Environment/figures/state_machine.tex <==
\begin{tikzpicture}[font=\footnotesize, scale=0.55]
 
% Start block
\node[draw,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1cm] (block1) {START};
 
% Voltage and Current Measurement
\node[draw,
    trapezium, 
    trapezium left angle = 65,
    trapezium right angle = 115,
    trapezium stretches,
    below=of block1,
    minimum width=3.5cm,
    minimum height=1cm
] (block2) { Measure $I_k$, $V_k$ };
 
% Power and voltage variation
\node[draw,
    below=of block2,
    minimum width=3.5cm,
    minimum height=1cm
] (block3) { $\Delta P=P_k-P_{k-1}$ \\ $\Delta V=V_k-V_{k-1}$};
 
% Conditions test
\node[draw,
    diamond,
    below=of block3,
    minimum width=2.5cm,
    inner sep=0] (block4) { $\Delta P>0$};
 
\node[draw,
    diamond,
    below left=of block4,
    minimum width=2.5cm,
    inner sep=0] (block5) { $\Delta V>0$};
 
\node[draw,
    diamond,
    below right=of block4,
    minimum width=2.5cm,
    inner sep=0] (block6) { $\Delta V>0$};
 
 
% Return block
\node[draw,
    rounded rectangle,
    below=5cm of block4,
    minimum width=2.5cm,
    minimum height=1cm,] (block11) { RETURN};
 
\node[coordinate,below=4.35cm of block4] (block12) {};
 
 
% Arrows
\draw[-latex] (block1) edge (block2)
    (block2) edge (block3)
    (block3) edge (block4);
 
\draw[-latex] (block4) -| (block5)
    node[pos=0.25,fill=white,inner sep=0]{Yes};
 
\draw[-latex] (block4) -| (block6)
    node[pos=0.25,fill=white,inner sep=0]{No};
 
 
\end{tikzpicture}

==> Soil_Sample_Search_in_a_Partially_Observable_Environment/packages.tex <==
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{algpseudocode}
\usepackage{tikz}
\usepackage{pgf-pie}  
\usetikzlibrary{shapes,positioning}
\usepackage{etoolbox}
\usepackage{afterpage,lipsum}
\usepackage{cite}
\usepackage{bm}
\usepackage{subcaption} %  for subfigures environments 


==> figures/state_machine.tex <==
\begin{tikzpicture}[font=\footnotesize, scale=0.55]
 
% Start block
\node[draw,
    rounded rectangle,
    minimum width=2.5cm,
    minimum height=1cm] (block1) {START};
 
% Voltage and Current Measurement
\node[draw,
    trapezium, 
    trapezium left angle = 65,
    trapezium right angle = 115,
    trapezium stretches,
    below=of block1,
    minimum width=3.5cm,
    minimum height=1cm
] (block2) { Measure $I_k$, $V_k$ };
 
% Power and voltage variation
\node[draw,
    below=of block2,
    minimum width=3.5cm,
    minimum height=1cm
] (block3) { $\Delta P=P_k-P_{k-1}$ \\ $\Delta V=V_k-V_{k-1}$};
 
% Conditions test
\node[draw,
    diamond,
    below=of block3,
    minimum width=2.5cm,
    inner sep=0] (block4) { $\Delta P>0$};
 
\node[draw,
    diamond,
    below left=of block4,
    minimum width=2.5cm,
    inner sep=0] (block5) { $\Delta V>0$};
 
\node[draw,
    diamond,
    below right=of block4,
    minimum width=2.5cm,
    inner sep=0] (block6) { $\Delta V>0$};
 
 
% Return block
\node[draw,
    rounded rectangle,
    below=5cm of block4,
    minimum width=2.5cm,
    minimum height=1cm,] (block11) { RETURN};
 
\node[coordinate,below=4.35cm of block4] (block12) {};
 
 
% Arrows
\draw[-latex] (block1) edge (block2)
    (block2) edge (block3)
    (block3) edge (block4);
 
\draw[-latex] (block4) -| (block5)
    node[pos=0.25,fill=white,inner sep=0]{Yes};
 
\draw[-latex] (block4) -| (block6)
    node[pos=0.25,fill=white,inner sep=0]{No};
 
 
\end{tikzpicture}
